Enhancing Multi-Scale Implicit Learning in Image Super-Resolution with Integrated Positional Encoding

Is the center position fully capable of representing a pixel? There is nothing wrong to represent pixels with their centers in a discrete image representation, but it makes more sense to consider each pixel as the aggregation of signals from a local area in an image super-resolution (SR) context. Despite the great capability of coordinate-based implicit representation in the field of arbitrary-scale image SR, this area's nature of pixels is not fully considered. To this end, we propose integrated positional encoding (IPE), extending traditional positional encoding by aggregating frequency information over the pixel area. We apply IPE to the state-of-the-art arbitrary-scale image super-resolution method: local implicit image function (LIIF), presenting IPE-LIIF. We show the effectiveness of IPE-LIIF by quantitative and qualitative evaluations, and further demonstrate the generalization ability of IPE to larger image scales and multiple implicit-based methods. Code will be released.

==> setup/package.tex <==

% Figures
\usepackage{graphicx}
\usepackage{subcaption}
\usepackage{float}
\usepackage[justification=raggedright]{caption}	% makes captions ragged right - thanks to Bryce Lobdell
\usepackage{lscape}                                         % Useful for wide tables or figures.
% \usepackage{wrapfig}
% \usepackage{authblk} % for double affiliations


\usepackage[symbol]{footmisc}
\renewcommand{\thefootnote}{\fnsymbol{footnote}}

% Algorithm
\usepackage[lined,ruled,linesnumbered]{algorithm2e}
\usepackage{animate} %% convert frames to video

% Table and list
\usepackage{booktabs}                   % Publication quality tables
\usepackage{multirow}

\usepackage{makecell}

\usepackage{paralist}
\usepackage{enumitem}

\usepackage[export]{adjustbox}

% Math
\usepackage{bm}                          % Make bold, italic math symbols
\usepackage{epsfig}                      % for figures
\usepackage{graphicx}                  % another package that works for figures
\usepackage{times}
\usepackage{mathptmx}
\usepackage{mathtools}
\usepackage{amssymb,amsmath}   % Short math guide for LaTeX ftp://ftp.ams.org/pub/tex/doc/amsmath/short-math-guide.pdf
\usepackage{breqn}

% Fonts
\usepackage{units}
\usepackage{color}

% Comments
\usepackage{comment}

% Hyperlinks
\usepackage{url}  % Hyphenation of URLs.
\usepackage[pagebackref=true,breaklinks=true,letterpaper=true,colorlinks,bookmarks=false]{hyperref}
% \usepackage{authblk}
% \usepackage{slashbox}
\usepackage{xspace}
\usepackage[table]{xcolor}
\usepackage{setspace}
\usepackage{grfext}
\PrependGraphicsExtensions*{.jpg,.png,.PNG}

\usepackage[T1]{fontenc}


% \usepackage{times,color}
% \usepackage{parskip}
% %\usepackage{epsfig}
% %\usepackage{psfig}
% %\usepackage[pdftex]{graphicx} % new acmsiggraph.cls
% \usepackage{ifthen}
% %\usepackage[draft]{hyperref} % new acmsiggraph.cls
% \usepackage{float}
% \usepackage{alltt}
% \usepackage{mathenv}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{amsthm}
% %\usepackage{rotating}
% \usepackage{newlfont} % for Box
% %\usepackage{ulem}
% \usepackage{floatflt}
% \usepackage{wrapfig}
% \usepackage{fixltx2e}
% \usepackage{subfig} % for subfloat
% \usepackage{multirow}
% \usepackage{cleveref}
% \usepackage{algorithmic}
% \usepackage{CJKutf8} % Chinese

